HandFlow: Quantifying View-Dependent 3D Ambiguity in Two-Hand Reconstruction with Normalizing Flow

Reconstructing two-hand interactions from a single image is a challenging problem due to ambiguities that stem from projective geometry and heavy occlusions. Existing methods are designed to estimate only a single pose, despite the fact that there exist other valid reconstructions that fit the image evidence equally well. In this paper we propose to address this issue by explicitly modeling the distribution of plausible reconstructions in a conditional normalizing flow framework. This allows us to directly supervise the posterior distribution through a novel determinant magnitude regularization, which is key to varied 3D hand pose samples that project well into the input image. We also demonstrate that metrics commonly used to assess reconstruction quality are insufficient to evaluate pose predictions under such severe ambiguity. To address this, we release the first dataset with multiple plausible annotations per image called MultiHands. The additional annotations enable us to evaluate the estimated distribution using the maximum mean discrepancy metric. Through this, we demonstrate the quality of our probabilistic reconstruction and show that explicit ambiguity modeling is better-suited for this challenging problem.

==> figures/TzionasFigure.tex <==
\begin{figure}
  \begin{subfigure}{0.32\columnwidth}
  \includegraphics[width=\linewidth]{figures/TzionasExamplesSkeleton/20_input.png}
  \end{subfigure}
  \begin{subfigure}{0.32\columnwidth}
  \includegraphics[width=\linewidth]{figures/TzionasExamplesSkeleton/20_fuzzy_0.png}
  \end{subfigure}
  \begin{subfigure}{0.32\columnwidth}
  \includegraphics[width=\linewidth]{figures/TzionasExamplesSkeleton/20_fuzzy_1.png}
  \end{subfigure}
  
  \begin{subfigure}{0.32\columnwidth}
  \includegraphics[width=\linewidth]{figures/TzionasExamplesSkeleton/40_input.png}
  \end{subfigure}
  \begin{subfigure}{0.32\columnwidth}
  \includegraphics[width=\linewidth]{figures/TzionasExamplesSkeleton/40_fuzzy_0.png}
  \end{subfigure}
  \begin{subfigure}{0.32\columnwidth}
  \includegraphics[width=\linewidth]{figures/TzionasExamplesSkeleton/40_fuzzy_1.png}
  \end{subfigure}
  
  \begin{subfigure}{0.32\columnwidth}
  \includegraphics[width=\linewidth]{figures/TzionasExamplesSkeleton/55_input.png}
  \end{subfigure}
  \begin{subfigure}{0.32\columnwidth}
  \includegraphics[width=\linewidth]{figures/TzionasExamplesSkeleton/55_fuzzy_0.png}
  \end{subfigure}
  \begin{subfigure}{0.32\columnwidth}
  \includegraphics[width=\linewidth]{figures/TzionasExamplesSkeleton/55_fuzzy_1.png}
  \end{subfigure}
    
  \begin{subfigure}{0.32\columnwidth}
  \includegraphics[width=\linewidth]{figures/TzionasExamplesSkeleton/76_input.png}
  \end{subfigure}
  \begin{subfigure}{0.32\columnwidth}
  \includegraphics[width=\linewidth]{figures/TzionasExamplesSkeleton/76_fuzzy_0.png}
  \end{subfigure}
  \begin{subfigure}{0.32\columnwidth}
  \includegraphics[width=\linewidth]{figures/TzionasExamplesSkeleton/76_fuzzy_1.png}
  \end{subfigure}
  
  \begin{subfigure}{0.32\columnwidth}
  \includegraphics[width=\linewidth]{figures/TzionasExamplesSkeleton/80_input.png}
  \end{subfigure}
  \begin{subfigure}{0.32\columnwidth}
  \includegraphics[width=\linewidth]{figures/TzionasExamplesSkeleton/80_fuzzy_0.png}
  \end{subfigure}
  \begin{subfigure}{0.32\columnwidth}
  \includegraphics[width=\linewidth]{figures/TzionasExamplesSkeleton/80_fuzzy_1.png}
  \end{subfigure}
    
  \begin{subfigure}{0.32\columnwidth}
  \includegraphics[width=\linewidth]{figures/TzionasExamplesSkeleton/100_input.png}
  \end{subfigure}
  \begin{subfigure}{0.32\columnwidth}
  \includegraphics[width=\linewidth]{figures/TzionasExamplesSkeleton/100_fuzzy_0.png}
  \end{subfigure}
  \begin{subfigure}{0.32\columnwidth}
  \includegraphics[width=\linewidth]{figures/TzionasExamplesSkeleton/100_fuzzy_1.png}
  \end{subfigure}
%
  
  \caption{Qualitative results on the Tzionas dataset \cite{tzionas_ijcv2016}. We demonstrate that our method can transfer the learned ability to handle 3D ambiguity to a different dataset, by using only 2D annotations.}
  \label{fig:tzionas}
\end{figure}


==> figures/annot_creation_pseudo_code.tex <==

\begin{algorithm}
 \KwData{Initial MANO Pose $\psi_{0}$}
 \KwResult{Additional annotations $\psi_{i}$}
 \BlankLine
 \tcp{Ensure: sampled $t \gets \{t_{right}, t_{left}\}$}
 \tcp{1. $\Delta P^{\text{2D}}(\psi_{i}(t)) < T$}
 \tcp{2. $\neg \text{collision}(\psi_{i}(t))$}
 \BlankLine
 $t \gets \text{sample\_translation}(\psi_{0})$\;
 $\psi_{i} \gets \text{update\_translation}(\psi_{0}, t)$\;
 \BlankLine
 
 \For{N iterations}{
 \BlankLine
  \tcp{Get finger with occluded joints:}
  \tcp{$\forall {P^{\text{3D}}_{j}} \in \{{P^{\text{3D}}}\}$}
  \tcp{$\text{child}({P^{\text{3D}}_{j}})$ are occluded}
  \BlankLine 
  $\{{P^{\text{3D}}}\} \gets \text{select\_finger}(\psi_{i})$\;

  $\psi_{i}' \gets \psi_{i}$
  \BlankLine
  \For{$P^{\text{3D}}_{j}$ in \{${P^{\text{3D}}}$\}}{
    \BlankLine
    \tcp{Ensure: sampled $Q^{\text{3D}}$}
    \tcp{1. $\text{bone}({Q^{\text{3D}}})$ = $\text{bone}({P^{\text{3D}}_{j}})$}
    \tcp{2. $Q^{\text{3D}}$ is occluded}
    \BlankLine
    
    $Q^{\text{3D}} \gets \text{sample\_joint}(P^{\text{3D}}_{j})$\;
    $\psi_{i}' = \text{update\_pose}(\psi_{i}', Q^{\text{3D}})$\;
    $\{{P^{\text{3D}}}\} = \text{update\_child}(\{{P^{\text{3D}}}\}, \psi_{i}')$\;
  }
  \BlankLine
  \tcp{likelihood from pose PCA}
  \If{$\text{is\_plausible}(\psi_{i}')$ }{
    $\psi_{i} \gets \psi_{i}'$ 
  }
 }
 \caption{\textit{Pseudocode for sampling additional annotations}}
 \label{alg:pseudo_code}
\end{algorithm}


==> figures/table_comparison_SoTA_abridged.tex <==
\begin{table}[t]
\begin{center}
{
\begin{tabular}{|l|ccc|}
\Xhline{2\arrayrulewidth}
Method &  Global  $\downarrow$ & RRR  $\downarrow$  & RR $\downarrow$ \\
%\hline\hline
\Xhline{2\arrayrulewidth}
Ours & \textbf{22.8} & \textbf{21.0} & \textbf{16.1}\\
Ours (Mode) & 51.4 & 30.7 & 18.2 \\
InterNet~\cite{moon2020interhand2} & 83.3 & 29.1 & 19.4 \\
Fan et al.~\cite{fan2021digit} & 81.7 & 32.1 & 17.2 \\
InterShape*~\cite{Zhang2021twohand} & - & 33.7 & 18.7\\
\Xhline{2\arrayrulewidth}%
\end{tabular}% 
}%
\end{center}
\caption{Our method produces samples that are on-par or better than the state-of-the-art methods. All results are in mm.
}

\label{table:comparisonSTAR_abridged}
\end{table}

==> supplementary_materials/AblationFigure.tex <==
\begin{figure}[hbt!]
  %
  \includegraphics[width=0.24\linewidth]{supplementary_materials/Ablation/1_400449_30765_0_ablated_orth.png}
  %
  \includegraphics[width=0.24\linewidth]{supplementary_materials/Ablation/1_400449_30765_1_ablated_orth.png}
  %
  \includegraphics[width=0.24\linewidth]{supplementary_materials/Ablation/1_400449_30765_2_ablated_orth.png}
  %
  \includegraphics[width=0.24\linewidth]{supplementary_materials/Ablation/1_400449_30765_3_ablated_orth.png}
  %

  %
  \includegraphics[width=0.24\linewidth]{supplementary_materials/Ablation/1_400449_30765_0_ablated_param.png}
  %
  \includegraphics[width=0.24\linewidth]{supplementary_materials/Ablation/1_400449_30765_1_ablated_param.png}
  %
  \includegraphics[width=0.24\linewidth]{supplementary_materials/Ablation/1_400449_30765_2_ablated_param.png}
  %
  \includegraphics[width=0.24\linewidth]{supplementary_materials/Ablation/1_400449_30765_3_ablated_param.png}
  
  \includegraphics[width=0.24\linewidth]{supplementary_materials/Ablation/1_400449_30765_0_ours.png}
  %
  \includegraphics[width=0.24\linewidth]{supplementary_materials/Ablation/1_400449_30765_1_ours.png}
  %
  \includegraphics[width=0.24\linewidth]{supplementary_materials/Ablation/1_400449_30765_2_ours.png}
  %
  \includegraphics[width=0.24\linewidth]{supplementary_materials/Ablation/1_400449_30765_3_ours.png}

  \caption{w/o $\mathcal{L}_{\text{Param}}$ (Top) and or w/o $\mathcal{L}_{\text{RotReg}}$ (Middle), ambiguity in joint supervision leads to unnatural twist rotations in samples. These ambiguities are reduced for our full method (Bottom).}
  \label{fig:ablation}
\end{figure}


==> supplementary_materials/FuzzyResults_new.tex <==
{
\newcommand{\ImageWidthSupp}{0.16}
\newcommand{\ImageHSepSupp}{0.1cm}
\newcommand{\ImageVSepSupp}{0.1cm}
\newcommand{\TitleVSepSupp}{0.35cm}
\begin{figure*}
  \centering
  \begin{tikzpicture}[every node/.style={inner sep=0,outer sep=0}]%
  % first row
  \node (image_IH_1_input) at (0,0) {\includegraphics[trim=0 1.2cm 0 1.2cm, clip, width=\ImageWidthSupp\linewidth]{supplementary_materials/FuzzyFigure/InterHand26M/107_input.png}};
  \node[above=\TitleVSepSupp of image_IH_1_input, anchor=north] {\small{Input}};
  \node[right=\ImageHSepSupp of image_IH_1_input, anchor=west] (image_IH_1_cam)  {\includegraphics[trim=2cm 1cm 2cm 1cm, clip, width=\ImageWidthSupp\linewidth]{supplementary_materials/FuzzyFigure/InterHand26M/107_000.png}};
  \node[above=\TitleVSepSupp of image_IH_1_cam, anchor=north] {\small{Camera View}};
  \node[right=\ImageHSepSupp of image_IH_1_cam, anchor=west] (image_IH_1_side) {\includegraphics[trim=2cm 1cm 2cm 1cm, clip, width=\ImageWidthSupp\linewidth]{supplementary_materials/FuzzyFigure/InterHand26M/107_283.png}};
  \node[above=\TitleVSepSupp of image_IH_1_side, anchor=north] {\small{Side View}};
  \node[right=\ImageHSepSupp of image_IH_1_side] (image_Tz_1_input) {\includegraphics[trim=0 1.2cm 0 1.2cm, clip, width=\ImageWidthSupp\linewidth]{supplementary_materials/FuzzyFigure/Tzionas/100_input.png}};
  \node[above=\TitleVSepSupp of image_Tz_1_input, anchor=north] {\small{Input}};
  \node[right=\ImageHSepSupp of image_Tz_1_input] (image_Tz_1_cam) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/FuzzyFigure/Tzionas/100_fuzzy_0.png}};
  \node[above=\TitleVSepSupp of image_Tz_1_cam, anchor=north] {\small{Camera View}};
  \node[right=\ImageHSepSupp of image_Tz_1_cam] (image_Tz_1_side) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/FuzzyFigure/Tzionas/100_fuzzy_1.png}};
  \node[above=\TitleVSepSupp of image_Tz_1_side, anchor=north] {\small{Side View}};
  %
  % second row
  \node[below=\ImageVSepSupp of image_IH_1_input, anchor=north] (image_IH_2_input) {\includegraphics[trim=0 1.2cm 0 1.2cm, clip, width=\ImageWidthSupp\linewidth]{supplementary_materials/FuzzyFigure/InterHand26M/2028_input.png}};
  \node[right=\ImageHSepSupp of image_IH_2_input, anchor=west] (image_IH_2_cam) {\includegraphics[trim=2cm 2cm 2cm 1cm, clip, width=\ImageWidthSupp\linewidth]{supplementary_materials/FuzzyFigure/InterHand26M/2028_000.png}};
  \node[right=\ImageHSepSupp of image_IH_2_cam, anchor=west] (image_IH_2_side) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/FuzzyFigure/InterHand26M/2028_107.png}};
  \node[right=\ImageHSepSupp of image_IH_2_side, anchor=west] (image_Tz_2_input) {\includegraphics[trim=0 1.2cm 0 1.2cm, clip, width=\ImageWidthSupp\linewidth]{supplementary_materials/FuzzyFigure/Tzionas/76_input.png}};
  \node[right=\ImageHSepSupp of image_Tz_2_input, anchor=west] (image_Tz_2_cam) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/FuzzyFigure/Tzionas/76_fuzzy_0.png}};
  \node[right=\ImageHSepSupp of image_Tz_2_cam, anchor=west] (image_Tz_2_side) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/FuzzyFigure/Tzionas/76_fuzzy_1.png}};
  %
  % third row
  \node[below=\ImageVSepSupp of image_IH_2_input, anchor=north] (image_IH_3_input) {\includegraphics[trim=0 1.2cm 0 1.2cm, clip, width=\ImageWidthSupp\linewidth]{supplementary_materials/FuzzyFigure/InterHand26M/2915_input.png}};
  \node[right=\ImageHSepSupp of image_IH_3_input, anchor=west] (image_IH_3_cam) {\includegraphics[trim=2cm 2cm 2cm 1cm, clip, width=\ImageWidthSupp\linewidth]{supplementary_materials/FuzzyFigure/InterHand26M/2915_000.png}};
  \node[right=\ImageHSepSupp of image_IH_3_cam, anchor=west] (image_IH_3_side) {\includegraphics[trim=2cm 2cm 2cm 1cm, clip, width=\ImageWidthSupp\linewidth]{supplementary_materials/FuzzyFigure/InterHand26M/2915_078.png}};
  \node[right=\ImageHSepSupp of image_IH_3_side, anchor=west] (image_Tz_3_input) {\includegraphics[trim=0 1.2cm 0 1.2cm, clip, width=\ImageWidthSupp\linewidth]{supplementary_materials/FuzzyFigure/Tzionas/80_input.png}};
  \node[right=\ImageHSepSupp of image_Tz_3_input, anchor=west] (image_Tz_3_cam) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/FuzzyFigure/Tzionas/80_fuzzy_0.png}};
  \node[right=\ImageHSepSupp of image_Tz_3_cam, anchor=west] (image_Tz_3_side) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/FuzzyFigure/Tzionas/80_fuzzy_1.png}};
  %
  % fourth row
  \node[below=\ImageVSepSupp of image_IH_3_input, anchor=north] (image_IH_4_input) {\includegraphics[trim=0 1.2cm 0 1.2cm, clip, width=\ImageWidthSupp\linewidth]{supplementary_materials/FuzzyFigure/InterHand26M/3096_input.png}};
  \node[right=\ImageHSepSupp of image_IH_4_input, anchor=west] (image_IH_4_cam) {\includegraphics[trim=2cm 2cm 2cm 1cm, clip, width=\ImageWidthSupp\linewidth]{supplementary_materials/FuzzyFigure/InterHand26M/3096_000.png}};
  \node[right=\ImageHSepSupp of image_IH_4_cam, anchor=west] (image_IH_4_side) {\includegraphics[trim=2cm 2cm 2cm 1cm, clip, width=\ImageWidthSupp\linewidth]{supplementary_materials/FuzzyFigure/InterHand26M/3096_139.png}};
  \node[right=\ImageHSepSupp of image_IH_4_side, anchor=west] (image_Tz_4_input) {\includegraphics[trim=0 1.2cm 0 1.2cm, clip, width=\ImageWidthSupp\linewidth]{supplementary_materials/FuzzyFigure/Tzionas/25_input.png}};
  \node[right=\ImageHSepSupp of image_Tz_4_input, anchor=west] (image_Tz_4_cam) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/FuzzyFigure/Tzionas/25_000.png}};
  \node[right=\ImageHSepSupp of image_Tz_4_cam, anchor=west] (image_Tz_4_side) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/FuzzyFigure/Tzionas/25_063.png}};
  %
  \end{tikzpicture}
  %
  \caption{
    We show 30 samples from the estimated distribution, rendered as semi-transparent skeletons, superimposed on a single image. These Samples are aligned to the root joint of one hand and the mode of the distribution is made opaque for ease of visualization. 
    Here we show more results from both the InterHand2.6M~\cite{moon2020interhand2} and the Tzionas~\cite{tzionas_ijcv2016} datasets.
  }
  \label{fig:FuzzySupp}
\end{figure*}
}

==> supplementary_materials/GroundTruthVis.tex <==
\newcommand{\ImageWidthGT}{0.118}
\newcommand{\ImageHSepGT}{0.05cm}
\newcommand{\ImageHSepGTH}{0.025cm}
\newcommand{\ImageVSepGT}{0.05cm}
\newcommand{\ImageBlockHSepGT}{0.2cm}
\newcommand{\ImageBlockVSepGT}{0.2cm}
\newcommand{\TitleHSepGT}{0.15cm}
\newcommand{\TitleVSepGT}{0.35cm}
\newcommand{\BoxThicknessGT}{semithick}
\begin{figure*}
  \centering
  \begin{tikzpicture}[every node/.style={inner sep=0,outer sep=0}]%
  % first row, left side
  \node (image_GT_1) at (0,0) {\includegraphics[trim={0 4cm 0 4cm},clip, width=\ImageWidthGT\linewidth]{supplementary_materials/GroundTruthVisualization/Capture0_ROM01_No_Interaction_2_Hand_cam400301_image20637/0.png}};
  \node[right=\ImageHSepGT of image_GT_1, anchor=west] (image_S_1_1) {\includegraphics[trim={0 4cm 0 4cm},clip, width=\ImageWidthGT\linewidth]{supplementary_materials/GroundTruthVisualization/Capture0_ROM01_No_Interaction_2_Hand_cam400301_image20637/1.png}};
  \node[right=\ImageHSepGT of image_S_1_1, anchor=west] (image_S_1_2) {\includegraphics[trim={0 4cm 0 4cm},clip, width=\ImageWidthGT\linewidth]{supplementary_materials/GroundTruthVisualization/Capture0_ROM01_No_Interaction_2_Hand_cam400301_image20637/5.png}};
  \node[right=\ImageHSepGT of image_S_1_2, anchor=west] (image_S_1_3)
  {\includegraphics[trim={0 4cm 0 4cm},clip, width=\ImageWidthGT\linewidth]{supplementary_materials/GroundTruthVisualization/Capture0_ROM01_No_Interaction_2_Hand_cam400301_image20637/9.png}};
  %
  % first row, right side
  \node[right=\ImageBlockHSepGT of image_S_1_3, anchor=west] (image_GT_2) {\includegraphics[trim={0 2cm 0 6cm},clip,width=\ImageWidthGT\linewidth]{supplementary_materials/GroundTruthVisualization/Capture0_ROM09_Interaction_Fingers_Touching_cam400416_image25077/0.png}};
  \node[right=\ImageHSepGT of image_GT_2, anchor=west] (image_S_2_1) {\includegraphics[trim={0 2cm 0 6cm},clip,width=\ImageWidthGT\linewidth]{supplementary_materials/GroundTruthVisualization/Capture0_ROM09_Interaction_Fingers_Touching_cam400416_image25077/2.png}};
  \node[right=\ImageHSepGT of image_S_2_1, anchor=west] (image_S_2_2) {\includegraphics[trim={0 2cm 0 6cm},clip,width=\ImageWidthGT\linewidth]{supplementary_materials/GroundTruthVisualization/Capture0_ROM09_Interaction_Fingers_Touching_cam400416_image25077/3.png}};
  \node[right=\ImageHSepGT of image_S_2_2, anchor=west] (image_S_2_3) {\includegraphics[trim={0 2cm 0 6cm},clip,width=\ImageWidthGT\linewidth]{supplementary_materials/GroundTruthVisualization/Capture0_ROM09_Interaction_Fingers_Touching_cam400416_image25077/8.png}};
  \node[left=\TitleHSepGT of image_GT_1, anchor=south, rotate=90] {\small{Cam View}};
  %
  % second row, left side
  \node[below=\ImageVSepGT of image_GT_1] (image_GT_1_novel) {\includegraphics[trim={0 4cm 0 4cm},clip, width=\ImageWidthGT\linewidth]{supplementary_materials/GroundTruthVisualization/Capture0_ROM01_No_Interaction_2_Hand_cam400301_image20637/side_013_0.png}};
  \node[right=\ImageHSepGT of image_GT_1_novel, anchor=west] (image_S_1_1_novel) {\includegraphics[trim={0 4cm 0 4cm},clip,width=\ImageWidthGT\linewidth]{supplementary_materials/GroundTruthVisualization/Capture0_ROM01_No_Interaction_2_Hand_cam400301_image20637/side_013_1.png}};
  \node[right=\ImageHSepGT of image_S_1_1_novel, anchor=west] (image_S_1_2_novel) {\includegraphics[trim={0 4cm 0 4cm},clip,width=\ImageWidthGT\linewidth]{supplementary_materials/GroundTruthVisualization/Capture0_ROM01_No_Interaction_2_Hand_cam400301_image20637/side_013_5.png}};
  \node[right=\ImageHSepGT of image_S_1_2_novel, anchor=west] (image_S_1_3_novel) {\includegraphics[trim={0 4cm 0 4cm},clip,width=\ImageWidthGT\linewidth]{supplementary_materials/GroundTruthVisualization/Capture0_ROM01_No_Interaction_2_Hand_cam400301_image20637/side_013_9.png}};
  %
  % second row, right side
  \node[right=\ImageBlockHSepGT of image_S_1_3_novel, anchor=west] (image_GT_2_novel) {\includegraphics[trim={0 3cm 0 5cm},clip,width=\ImageWidthGT\linewidth]{supplementary_materials/GroundTruthVisualization/Capture0_ROM09_Interaction_Fingers_Touching_cam400416_image25077/side_005_0.png}};
  \node[right=\ImageHSepGT of image_GT_2_novel, anchor=west] (image_S_2_1_novel) {\includegraphics[trim={0 3cm 0 5cm},clip,width=\ImageWidthGT\linewidth]{supplementary_materials/GroundTruthVisualization/Capture0_ROM09_Interaction_Fingers_Touching_cam400416_image25077/side_005_2.png}};
  \node[right=\ImageHSepGT of image_S_2_1_novel, anchor=west] (image_S_2_2_novel) {\includegraphics[trim={0 3cm 0 5cm},clip,width=\ImageWidthGT\linewidth]{supplementary_materials/GroundTruthVisualization/Capture0_ROM09_Interaction_Fingers_Touching_cam400416_image25077/side_005_3.png}};
  \node[right=\ImageHSepGT of image_S_2_2_novel, anchor=west] (image_S_2_3_novel) {\includegraphics[trim={0 3cm 0 5cm},clip,width=\ImageWidthGT\linewidth]{supplementary_materials/GroundTruthVisualization/Capture0_ROM09_Interaction_Fingers_Touching_cam400416_image25077/side_005_8.png}};
  \node[left=\TitleHSepGT of image_GT_1_novel, anchor=south, rotate=90] {\small{Novel View}};
  %
  % third row, left side
  \node[below=\ImageVSepGT of image_GT_1_novel] (image_GT_3) {\includegraphics[trim={0 4cm 0 4cm},clip, width=\ImageWidthGT\linewidth]{supplementary_materials/GroundTruthVisualization/Capture1_ROM09_Interaction_Fingers_Touching_cam400312_image31059/0.png}};
  \node[right=\ImageHSepGT of image_GT_3, anchor=west] (image_S_3_1) {\includegraphics[trim={0 4cm 0 4cm},clip, width=\ImageWidthGT\linewidth]{supplementary_materials/GroundTruthVisualization/Capture1_ROM09_Interaction_Fingers_Touching_cam400312_image31059/5.png}};
  \node[right=\ImageHSepGT of image_S_3_1, anchor=west] (image_S_3_2) {\includegraphics[trim={0 4cm 0 4cm},clip, width=\ImageWidthGT\linewidth]{supplementary_materials/GroundTruthVisualization/Capture1_ROM09_Interaction_Fingers_Touching_cam400312_image31059/6.png}};
  \node[right=\ImageHSepGT of image_S_3_2, anchor=west] (image_S_3_3)
  {\includegraphics[trim={0 4cm 0 4cm},clip, width=\ImageWidthGT\linewidth]{supplementary_materials/GroundTruthVisualization/Capture1_ROM09_Interaction_Fingers_Touching_cam400312_image31059/10.png}};
  %
  % third row, right side
  \node[right=\ImageBlockHSepGT of image_S_3_3, anchor=west] (image_GT_4) {\includegraphics[trim={0 2cm 0 6cm},clip,width=\ImageWidthGT\linewidth]{supplementary_materials/GroundTruthVisualization/Capture1_ROM09_Interaction_Fingers_Touching_cam400421_image30207/0.png}};
  \node[right=\ImageHSepGT of image_GT_4, anchor=west] (image_S_4_1) {\includegraphics[trim={0 2cm 0 6cm},clip,width=\ImageWidthGT\linewidth]{supplementary_materials/GroundTruthVisualization/Capture1_ROM09_Interaction_Fingers_Touching_cam400421_image30207/2.png}};
  \node[right=\ImageHSepGT of image_S_4_1, anchor=west] (image_S_4_2) {\includegraphics[trim={0 2cm 0 6cm},clip,width=\ImageWidthGT\linewidth]{supplementary_materials/GroundTruthVisualization/Capture1_ROM09_Interaction_Fingers_Touching_cam400421_image30207/7.png}};
  \node[right=\ImageHSepGT of image_S_4_2, anchor=west] (image_S_4_3) {\includegraphics[trim={0 2cm 0 6cm},clip,width=\ImageWidthGT\linewidth]{supplementary_materials/GroundTruthVisualization/Capture1_ROM09_Interaction_Fingers_Touching_cam400421_image30207/10.png}};
  \node[left=\TitleHSepGT of image_GT_3, anchor=south, rotate=90] {\small{Cam View}};
  %
  % fourth row, left side
  \node[below=\ImageVSepGT of image_GT_3] (image_GT_3_novel) {\includegraphics[trim={0 4cm 0 4cm},clip, width=\ImageWidthGT\linewidth]{supplementary_materials/GroundTruthVisualization/Capture1_ROM09_Interaction_Fingers_Touching_cam400312_image31059/side_003_0.png}};
  \node[right=\ImageHSepGT of image_GT_3_novel, anchor=west] (image_S_3_1_novel) {\includegraphics[trim={0 4cm 0 4cm},clip,width=\ImageWidthGT\linewidth]{supplementary_materials/GroundTruthVisualization/Capture1_ROM09_Interaction_Fingers_Touching_cam400312_image31059/side_003_5.png}};
  \node[right=\ImageHSepGT of image_S_3_1_novel, anchor=west] (image_S_3_2_novel) {\includegraphics[trim={0 4cm 0 4cm},clip,width=\ImageWidthGT\linewidth]{supplementary_materials/GroundTruthVisualization/Capture1_ROM09_Interaction_Fingers_Touching_cam400312_image31059/side_003_6.png}};
  \node[right=\ImageHSepGT of image_S_3_2_novel, anchor=west] (image_S_3_3_novel) {\includegraphics[trim={0 4cm 0 4cm},clip,width=\ImageWidthGT\linewidth]{supplementary_materials/GroundTruthVisualization/Capture1_ROM09_Interaction_Fingers_Touching_cam400312_image31059/side_003_10.png}};
  %
  % fourth row, right side
  \node[right=\ImageBlockHSepGT of image_S_3_3_novel, anchor=west] (image_GT_4_novel) {\includegraphics[trim={0 3cm 0 5cm},clip,width=\ImageWidthGT\linewidth]{supplementary_materials/GroundTruthVisualization/Capture1_ROM09_Interaction_Fingers_Touching_cam400421_image30207/side_005_0.png}};
  \node[right=\ImageHSepGT of image_GT_4_novel, anchor=west] (image_S_4_1_novel) {\includegraphics[trim={0 3cm 0 5cm},clip,width=\ImageWidthGT\linewidth]{supplementary_materials/GroundTruthVisualization/Capture1_ROM09_Interaction_Fingers_Touching_cam400421_image30207/side_005_2.png}};
  \node[right=\ImageHSepGT of image_S_4_1_novel, anchor=west] (image_S_4_2_novel) {\includegraphics[trim={0 3cm 0 5cm},clip,width=\ImageWidthGT\linewidth]{supplementary_materials/GroundTruthVisualization/Capture1_ROM09_Interaction_Fingers_Touching_cam400421_image30207/side_005_7.png}};
  \node[right=\ImageHSepGT of image_S_4_2_novel, anchor=west] (image_S_4_3_novel) {\includegraphics[trim={0 3cm 0 5cm},clip,width=\ImageWidthGT\linewidth]{supplementary_materials/GroundTruthVisualization/Capture1_ROM09_Interaction_Fingers_Touching_cam400421_image30207/side_005_10.png}};
  \node[left=\TitleHSepGT of image_GT_3_novel, anchor=south, rotate=90] {\small{Novel View}};
  %
  % fifth row, left side
  \node[below=\ImageVSepGT of image_GT_3_novel] (image_GT_5) {\includegraphics[trim={0 4cm 0 4cm},clip, width=\ImageWidthGT\linewidth]{supplementary_materials/GroundTruthVisualization/Capture6_0275_leftbabybird_cam410238_image48011/0.png}};
  \node[right=\ImageHSepGT of image_GT_5, anchor=west] (image_S_5_1) {\includegraphics[trim={0 4cm 0 4cm},clip, width=\ImageWidthGT\linewidth]{supplementary_materials/GroundTruthVisualization/Capture6_0275_leftbabybird_cam410238_image48011/2.png}};
  \node[right=\ImageHSepGT of image_S_5_1, anchor=west] (image_S_5_2) {\includegraphics[trim={0 4cm 0 4cm},clip, width=\ImageWidthGT\linewidth]{supplementary_materials/GroundTruthVisualization/Capture6_0275_leftbabybird_cam410238_image48011/3.png}};
  \node[right=\ImageHSepGT of image_S_5_2, anchor=west] (image_S_5_3)
  {\includegraphics[trim={0 4cm 0 4cm},clip, width=\ImageWidthGT\linewidth]{supplementary_materials/GroundTruthVisualization/Capture6_0275_leftbabybird_cam410238_image48011/7.png}};
  %
  % fifth row, right side
  \node[right=\ImageBlockHSepGT of image_S_5_3, anchor=west] (image_GT_6) {\includegraphics[trim={0 2cm 0 6cm},clip,width=\ImageWidthGT\linewidth]{supplementary_materials/GroundTruthVisualization/Capture1_ROM09_Interaction_Fingers_Touching_cam400283_image29679/0.png}};
  \node[right=\ImageHSepGT of image_GT_6, anchor=west] (image_S_6_1) {\includegraphics[trim={0 2cm 0 6cm},clip,width=\ImageWidthGT\linewidth]{supplementary_materials/GroundTruthVisualization/Capture1_ROM09_Interaction_Fingers_Touching_cam400283_image29679/2.png}};
  \node[right=\ImageHSepGT of image_S_6_1, anchor=west] (image_S_6_2) {\includegraphics[trim={0 2cm 0 6cm},clip,width=\ImageWidthGT\linewidth]{supplementary_materials/GroundTruthVisualization/Capture1_ROM09_Interaction_Fingers_Touching_cam400283_image29679/5.png}};
  \node[right=\ImageHSepGT of image_S_6_2, anchor=west] (image_S_6_3) {\includegraphics[trim={0 2cm 0 6cm},clip,width=\ImageWidthGT\linewidth]{supplementary_materials/GroundTruthVisualization/Capture1_ROM09_Interaction_Fingers_Touching_cam400283_image29679/6.png}};
  \node[left=\TitleHSepGT of image_GT_5, anchor=south, rotate=90] {\small{Cam View}};
  %
  % sixth row, left side
  \node[below=\ImageVSepGT of image_GT_5] (image_GT_5_novel) {\includegraphics[trim={0 4cm 0 4cm},clip, width=\ImageWidthGT\linewidth]{supplementary_materials/GroundTruthVisualization/Capture6_0275_leftbabybird_cam410238_image48011/side_005_0.png}};
  \node[right=\ImageHSepGT of image_GT_5_novel, anchor=west] (image_S_5_1_novel) {\includegraphics[trim={0 4cm 0 4cm},clip,width=\ImageWidthGT\linewidth]{supplementary_materials/GroundTruthVisualization/Capture6_0275_leftbabybird_cam410238_image48011/side_005_2.png}};
  \node[right=\ImageHSepGT of image_S_5_1_novel, anchor=west] (image_S_5_2_novel) {\includegraphics[trim={0 4cm 0 4cm},clip,width=\ImageWidthGT\linewidth]{supplementary_materials/GroundTruthVisualization/Capture6_0275_leftbabybird_cam410238_image48011/side_005_3.png}};
  \node[right=\ImageHSepGT of image_S_5_2_novel, anchor=west] (image_S_5_3_novel) {\includegraphics[trim={0 4cm 0 4cm},clip,width=\ImageWidthGT\linewidth]{supplementary_materials/GroundTruthVisualization/Capture6_0275_leftbabybird_cam410238_image48011/side_005_7.png}};
  %
  % sixth row, right side
  \node[right=\ImageBlockHSepGT of image_S_5_3_novel, anchor=west] (image_GT_6_novel) {\includegraphics[trim={0 3cm 0 5cm},clip,width=\ImageWidthGT\linewidth]{supplementary_materials/GroundTruthVisualization/Capture1_ROM09_Interaction_Fingers_Touching_cam400283_image29679/side_004_0.png}};
  \node[right=\ImageHSepGT of image_GT_6_novel, anchor=west] (image_S_6_1_novel) {\includegraphics[trim={0 3cm 0 5cm},clip,width=\ImageWidthGT\linewidth]{supplementary_materials/GroundTruthVisualization/Capture1_ROM09_Interaction_Fingers_Touching_cam400283_image29679/side_004_2.png}};
  \node[right=\ImageHSepGT of image_S_6_1_novel, anchor=west] (image_S_6_2_novel) {\includegraphics[trim={0 3cm 0 5cm},clip,width=\ImageWidthGT\linewidth]{supplementary_materials/GroundTruthVisualization/Capture1_ROM09_Interaction_Fingers_Touching_cam400283_image29679/side_004_5.png}};
  \node[right=\ImageHSepGT of image_S_6_2_novel, anchor=west] (image_S_6_3_novel) {\includegraphics[trim={0 3cm 0 5cm},clip,width=\ImageWidthGT\linewidth]{supplementary_materials/GroundTruthVisualization/Capture1_ROM09_Interaction_Fingers_Touching_cam400283_image29679/side_004_6.png}};
  \node[left=\TitleHSepGT of image_GT_5_novel, anchor=south, rotate=90] {\small{Novel View}};

  \foreach \i in {1,...,6}
  {
  \node[draw,\BoxThicknessGT,fit=(image_GT_\i_novel)] {};
  \node[draw,\BoxThicknessGT,fit=(image_S_\i_3_novel)] {};
  \node[draw,\BoxThicknessGT,fit=(image_S_\i_1_novel)] {};
  \node[draw,\BoxThicknessGT,fit=(image_S_\i_1_novel) (image_S_\i_2_novel) (image_S_\i_3_novel)] {};
  
  \node[draw,\BoxThicknessGT,fit=(image_GT_\i)] {};
  \node[draw,\BoxThicknessGT,fit=(image_S_\i_3)] {};
  \node[draw,\BoxThicknessGT,fit=(image_S_\i_1)] {};
  \node[draw,\BoxThicknessGT,fit=(image_S_\i_1) (image_S_\i_2) (image_S_\i_3)] {};
  }
  \end{tikzpicture}

  \caption{More visualizations of the our MultiHands dataset. Note the diversity of 3D poses that can be seen in the novel view. 
  }
  \label{fig:gt_vis_sup}
\end{figure*}


==> supplementary_materials/OverlayResults_new.tex <==
{
\newcommand{\ImageWidthSupp}{0.118}
\newcommand{\ImageHSepSupp}{0.05cm}
\newcommand{\ImageVSepSupp}{0.05cm}
\newcommand{\ImageBlockHSepSupp}{0.2cm}
\newcommand{\ImageBlockVSepSupp}{0.2cm}
\newcommand{\TitleHSepSupp}{0.15cm}
\newcommand{\TitleVSepSupp}{0.35cm}
%
\newcommand{\BoxThicknessSupp}{semithick}
\begin{figure*}
  \centering
  \begin{tikzpicture}[every node/.style={inner sep=0,outer sep=0}]%
  % first row, left side
  \node (image_GT_1) at (0,0) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/355_gt_joints.png}};
  \node[above=\TitleVSepSupp of image_GT_1, anchor=north] {\small{Ground Truth}};
  \node[right=\ImageHSepSupp of image_GT_1, anchor=west] (image_S_1_1) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/355_1.png}};
  \node[right=\ImageHSepSupp of image_S_1_1, anchor=west] (image_S_1_2) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/355_3.png}};
  \node[above=\TitleVSepSupp of image_S_1_2, anchor=north] {\small{Our Samples}};
  \node[right=\ImageHSepSupp of image_S_1_2, anchor=west] (image_S_1_3) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/355_4.png}};
  %
  % first row, right side
  \node[right=\ImageBlockHSepSupp of image_S_1_3, anchor=west] (image_GT_2) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/370_gt_joints.png}};
  \node[above=\TitleVSepSupp of image_GT_2, anchor=north] {\small{Ground Truth}};
  \node[right=\ImageHSepSupp of image_GT_2, anchor=west] (image_S_2_1) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/370_0.png}};
  \node[right=\ImageHSepSupp of image_S_2_1, anchor=west] (image_S_2_2) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/370_1.png}};
  \node[above=\TitleVSepSupp of image_S_2_2, anchor=north] {\small{Our Samples}};
  \node[right=\ImageHSepSupp of image_S_2_2, anchor=west] (image_S_2_3) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/370_3.png}};
  \node[left=\TitleHSepSupp of image_GT_1, anchor=south, rotate=90] {\small{Cam View}};
  %
  % second row, left side
  \node[below=\ImageVSepSupp of image_GT_1] (image_GT_1_novel) {\includegraphics[trim={0 0cm 0 1cm},clip, width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/355_gt_041.png}};
  \node[right=\ImageHSepSupp of image_GT_1_novel, anchor=west] (image_S_1_1_novel) {\includegraphics[trim={0 0cm 0 1cm},clip,width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/355_1_041.png}};
  \node[right=\ImageHSepSupp of image_S_1_1_novel, anchor=west] (image_S_1_2_novel) {\includegraphics[trim={0 0cm 0 1cm},clip,width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/355_3_041.png}};
  \node[right=\ImageHSepSupp of image_S_1_2_novel, anchor=west] (image_S_1_3_novel) {\includegraphics[trim={0 0cm 0 1cm},clip,width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/355_4_041.png}};
  %
  % second row, right side
  \node[right=\ImageBlockHSepSupp of image_S_1_3_novel, anchor=west] (image_GT_2_novel) {\includegraphics[trim={0 0cm 0 1cm},clip,width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/370_gt_066.png}};
  \node[right=\ImageHSepSupp of image_GT_2_novel, anchor=west] (image_S_2_1_novel) {\includegraphics[trim={0 0cm 0 1cm},clip,width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/370_0_066.png}};
  \node[right=\ImageHSepSupp of image_S_2_1_novel, anchor=west] (image_S_2_2_novel) {\includegraphics[trim={0 0cm 0 1cm},clip,width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/370_1_066.png}};
  \node[right=\ImageHSepSupp of image_S_2_2_novel, anchor=west] (image_S_2_3_novel) {\includegraphics[trim={0 0cm 0 1cm},clip,width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/370_3_066.png}};
  \node[left=\TitleHSepSupp of image_GT_1_novel, anchor=south, rotate=90] {\small{Novel View}};
  %
  % third row, left side
  \node[below=\ImageBlockVSepSupp of image_GT_1_novel] (image_GT_3) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/210_gt_joints.png}};
  \node[right=\ImageHSepSupp of image_GT_3, anchor=west] (image_S_3_1) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/210_0.png}};
  \node[right=\ImageHSepSupp of image_S_3_1, anchor=west] (image_S_3_2) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/210_2.png}};
  \node[right=\ImageHSepSupp of image_S_3_2, anchor=west] (image_S_3_3) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/210_3.png}};
  %
  % third row, right side
  \node[right=\ImageBlockHSepSupp of image_S_3_3, anchor=west] (image_GT_4) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/399_gt_joints.png}};
  \node[right=\ImageHSepSupp of image_GT_4, anchor=west] (image_S_4_1) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/399_0.png}};
  \node[right=\ImageHSepSupp of image_S_4_1, anchor=west] (image_S_4_2) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/399_1.png}};
  \node[right=\ImageHSepSupp of image_S_4_2, anchor=west] (image_S_4_3) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/399_3.png}};
  \node[left=\TitleHSepSupp of image_GT_3, anchor=south, rotate=90] {\small{Cam View}};
  %
  % fourth row, left side
  \node[below=\ImageVSepSupp of image_GT_3] (image_GT_3_novel) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/210_gt_024.png}};
  \node[right=\ImageHSepSupp of image_GT_3_novel, anchor=west] (image_S_3_1_novel) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/210_0_024.png}};
  \node[right=\ImageHSepSupp of image_S_3_1_novel, anchor=west] (image_S_3_2_novel) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/210_2_024.png}};
  \node[right=\ImageHSepSupp of image_S_3_2_novel, anchor=west] (image_S_3_3_novel) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/210_3_024.png}};
  %
  % fourth row, right side
  \node[right=\ImageBlockHSepSupp of image_S_3_3_novel, anchor=west] (image_GT_4_novel) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/399_gt_220.png}};
  \node[right=\ImageHSepSupp of image_GT_4_novel, anchor=west] (image_S_4_1_novel) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/399_0_220.png}};
  \node[right=\ImageHSepSupp of image_S_4_1_novel, anchor=west] (image_S_4_2_novel) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/399_1_220.png}};
  \node[right=\ImageHSepSupp of image_S_4_2_novel, anchor=west] (image_S_4_3_novel) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/399_3_220.png}};
  \node[left=\TitleHSepSupp of image_GT_3_novel, anchor=south, rotate=90] {\small{Novel View}};
  %
  % fifth row, left side
  \node[below=\ImageBlockVSepSupp of image_GT_3_novel] (image_GT_5) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/752_gt_joints.png}};
  \node[right=\ImageHSepSupp of image_GT_5, anchor=west] (image_S_5_1) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/752_0.png}};
  \node[right=\ImageHSepSupp of image_S_5_1, anchor=west] (image_S_5_2) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/752_1.png}};
  \node[right=\ImageHSepSupp of image_S_5_2, anchor=west] (image_S_5_3) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/752_4.png}};
  %
  % fifth row, right side
  \node[right=\ImageBlockHSepSupp of image_S_5_3, anchor=west] (image_GT_6) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/1087_gt_joints.png}};
  \node[right=\ImageHSepSupp of image_GT_6, anchor=west] (image_S_6_1) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/1087_1.png}};
  \node[right=\ImageHSepSupp of image_S_6_1, anchor=west] (image_S_6_2) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/1087_2.png}};
  \node[right=\ImageHSepSupp of image_S_6_2, anchor=west] (image_S_6_3) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/1087_4.png}};
  \node[left=\TitleHSepSupp of image_GT_5, anchor=south, rotate=90] {\small{Cam View}};
  %
  % sixth row, left side
  \node[below=\ImageVSepSupp of image_GT_5] (image_GT_5_novel) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/752_gt_108.png}};
  \node[right=\ImageHSepSupp of image_GT_5_novel, anchor=west] (image_S_5_1_novel) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/752_0_108.png}};
  \node[right=\ImageHSepSupp of image_S_5_1_novel, anchor=west] (image_S_5_2_novel) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/752_1_108.png}};
  \node[right=\ImageHSepSupp of image_S_5_2_novel, anchor=west] (image_S_5_3_novel) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/752_4_108.png}};
  %
  % sixth row, right side
  \node[right=\ImageBlockHSepSupp of image_S_5_3_novel, anchor=west] (image_GT_6_novel) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/1087_gt_071.png}};
  \node[right=\ImageHSepSupp of image_GT_6_novel, anchor=west] (image_S_6_1_novel) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/1087_1_071.png}};
  \node[right=\ImageHSepSupp of image_S_6_1_novel, anchor=west] (image_S_6_2_novel) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/1087_2_071.png}};
  \node[right=\ImageHSepSupp of image_S_6_2_novel, anchor=west] (image_S_6_3_novel) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/1087_4_071.png}};
  \node[left=\TitleHSepSupp of image_GT_5_novel, anchor=south, rotate=90] {\small{Novel View}};
  %
  % seventh row, left side
  \node[below=\ImageBlockVSepSupp of image_GT_5_novel] (image_GT_7)
  {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/1111_gt_joints.png}};
  \node[right=\ImageHSepSupp of image_GT_7, anchor=west] (image_S_7_1)
  {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/1111_0.png}};
  \node[right=\ImageHSepSupp of image_S_7_1, anchor=west] (image_S_7_2)
  {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/1111_1.png}};
  \node[right=\ImageHSepSupp of image_S_7_2, anchor=west] (image_S_7_3)
  {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/1111_3.png}};
  %
  % seventh row, right side
  \node[right=\ImageBlockHSepSupp of image_S_7_3, anchor=west] (image_GT_8)
  {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/2024_gt_joints.png}};
  \node[right=\ImageHSepSupp of image_GT_8, anchor=west] (image_S_8_1)
  {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/2024_1.png}};
  \node[right=\ImageHSepSupp of image_S_8_1, anchor=west] (image_S_8_2)
  {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/2024_18.png}};
  \node[right=\ImageHSepSupp of image_S_8_2, anchor=west] (image_S_8_3)
  {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/2024_24.png}};
  \node[left=\TitleHSepSupp of image_GT_7, anchor=south, rotate=90] {\small{Cam View}};
  %
  % eight row, left side
  \node[below=\ImageVSepSupp of image_GT_7] (image_GT_7_novel) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/1111_gt_080.png}};
  \node[right=\ImageHSepSupp of image_GT_7_novel, anchor=west] (image_S_7_1_novel) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/1111_0_080.png}};
  \node[right=\ImageHSepSupp of image_S_7_1_novel, anchor=west] (image_S_7_2_novel) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/1111_1_080.png}};
  \node[right=\ImageHSepSupp of image_S_7_2_novel, anchor=west] (image_S_7_3_novel) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/1111_3_080.png}};
  %
  % eight row, right side
  \node[right=\ImageBlockHSepSupp of image_S_7_3_novel, anchor=west] (image_GT_8_novel) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/2024_gt_100.png}};
  \node[right=\ImageHSepSupp of image_GT_8_novel, anchor=west] (image_S_8_1_novel) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/2024_1_100.png}};
  \node[right=\ImageHSepSupp of image_S_8_1_novel, anchor=west] (image_S_8_2_novel) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/2024_18_100.png}};
  \node[right=\ImageHSepSupp of image_S_8_2_novel, anchor=west] (image_S_8_3_novel) {\includegraphics[width=\ImageWidthSupp\linewidth]{supplementary_materials/OverlayResults/InterHand26M/2024_24_100.png}};
  \node[left=\TitleHSepSupp of image_GT_7_novel, anchor=south, rotate=90] {\small{Novel View}};
  \vspace{-0.3cm}
  % boxes
  \foreach \i in {1,...,8}
  {
  \node[draw,\BoxThicknessSupp,fit=(image_GT_\i_novel)] {};
  \node[draw,dash dot dot,\BoxThicknessSupp,fit=(image_S_\i_2_novel)] {};
  \node[draw,\BoxThicknessSupp,fit=(image_S_\i_1_novel) (image_S_\i_2_novel) (image_S_\i_3_novel)] {};
  }
  \end{tikzpicture}
  
  \caption{We show more individual mesh samples from the camera view and from a novel view. Note that not all joints are annotated in the ground truth. This shows up as missing segments in the skeleton.}
  \label{figure:OverlaySupp}
\end{figure*}
}

